On Interactive Coding Schemes with Adaptive Termination

In interactive coding, Alice and Bob wish to compute some function $f$ of their individual private inputs $x$ and $y$. They do this by engaging in an interactive protocol to jointly compute $f(x,y)$. The goal is to do this in an error-resilient way, such that even given some fraction of adversarial corruptions to the protocol, both parties still learn $f(x,y)$. Typically, the error resilient protocols constructed by interactive coding schemes are \emph{non-adaptive}, that is, the length of the protocol as well as the speaker in each round is fixed beforehand. The maximal error resilience obtainable by non-adaptive schemes is now well understood. In order to circumvent known barriers and achieve higher error resilience, the work of Agrawal, Gelles, and Sahai (ISIT 2016) introduced to interactive coding the notion of \emph{adaptive} schemes, where the length of the protocol or the speaker order are no longer necessarily fixed. In this paper, we study the power of \emph{adaptive termination} in the context of the error resilience of interactive coding schemes. In other words, what is the power of schemes where Alice and Bob are allowed to disengage from the protocol early? We study this question in two contexts, both for the task of \emph{message exchange}, where the goal is to learn the other party's input.

==> 1termination.tex <==
\section{Noise Rate Relative to First Termination}

\begin{definition}
    The \emph{noise rate relative to the first termination} is the fraction of corrupted rounds out of the number of rounds until \emph{either} party terminates. 
\end{definition}

Under this noise rate definition, at any point, either party can choose to fully determine the adversary's budget by terminating. Once a party has terminated, the adversary gains no additional budget from the extra rounds the other party stays in for. Intuitively, this model has the strongest parties and the weakest adversary, and should be able to tolerate the highest rate of noise.

This is indeed the case. For any $\epsilon > 0$, we demonstrate a protocol that is resilient to a $(\frac12 - \epsilon)$-fraction of noise. The protocol, described in Figure~\ref{fig:1termination-1/2}, occurs in \emph{batches}, which are a set of consecutive rounds where the same party speaks in all the rounds. We say that a party that speaks in a batch sends $m \in \Sigma^\ell$ if they send the $\ell$ characters of $m$ in the next $\ell$ rounds.
\ynote{We should consider $\Sigma=\{0,1\}$, in which case we get resilience to $1/4-\epsilon$ error, which is the best in this setting?}
\begin{figure}[h!]
    \centering
    \protocol{}{
        Let $C_\epsilon = \frac1\epsilon-1$.
        \begin{enumerate}\setcounter{enumi}{-1}
        \item 
            Alice and Bob decide on a family of codes $\ECC_i : \{ 0, 1 \}^{n_A} \rightarrow \Sigma^{N_i}$, with $|\Sigma| = O(1)$. Each $\ECC_i$ has a relative distance of $1 - \epsilon$ and length $N_i = C_\epsilon^{2i} \cdot N$.
        \item 
            In batch $2k$, $k \ge 0$, Alice encodes $x$ via $\ECC_k$ of length $N_k$ to get $\hat{x}_k$ and sends $\hat{x}_k$ to Bob. 
            
            When $k \ge 1$, if at least half of the characters in $\hat{y}_{k-1}$ are not $0$'s, Alice terminates and outputs $(x, k-1)$.
        \item 
            In batch $2k + 1$, $k \ge 0$, if $k < y$ (we interpret Bob's input $y$ as a number between $0$ and $2^{n_B}-1$ inclusive), Bob sends Alice $\hat{y}_k = 0^{C_\epsilon \cdot N_k}$. Otherwise, if $k = y$, Bob terminates and outputs $(\DEC(\hat{x}_k), y)$.
        \end{enumerate}
    }
    \caption{Adaptive length coding scheme with resilience $\frac12$ in the first termination model}
    \label{fig:1termination-1/2}
\end{figure}

\begin{theorem}
    The protocol in Figure~\ref{fig:1termination-1/2} is resilient to a $(\frac12-\epsilon)$-fraction of noise computed relative to the first party termination. \rnote{add comment about rate? doubly exponential in $n_B$}
\end{theorem}

\begin{proof}
    First, note that the number of messages sent in batch $j$ is $C_\epsilon^j \cdot N$. This means that the total number of messages sent in the first $j$ batches is $N(1 + C_\epsilon + \dots + C_\epsilon^j) = N \cdot \frac{C_\epsilon^{j+1}-1}{C_\epsilon-1}$. 
    
    We split the analysis into cases:
    \begin{itemize}
    \item First, in the case that Alice terminates before Bob does, it must be the case that the adversary corrupted at least half of the symbols in Bob's most recent message $\hat{y}_{k-1}$. Then, the noise rate computed relative to Alice's termination is 
    \[
        \ge \frac{\frac12 C_\epsilon^{2k-1} N}{(C_\epsilon^{2k}-1)/(C_\epsilon-1) \cdot N}
        > \frac{\frac12 (C_\epsilon-1) \cdot C_\epsilon^{2k-1}}{C_\epsilon^{2k}}
        \ge \frac12 \cdot \frac{\frac1\epsilon-2}{\frac1\epsilon-1}
        \ge \frac12 \cdot \frac{\frac1\epsilon-2}{\frac1\epsilon}
        = \frac12 - \epsilon.
    \]
    \item Otherwise, suppose that Bob terminates before Alice does. This means that Bob terminates at the beginning of batch $2y+1$. If Bob outputs the wrong value, it means that $\DEC(\hat{x}_y) \not= x$, and at least $\frac{1-\epsilon}2$ of the bits in $\hat{x}_y$ were changed. This gives a noise rate of 
    \[
        \ge \frac{\frac{1-\epsilon}2 \cdot C_\epsilon^{2y} N}{(C_\epsilon^{2y+1}-1)/(C_\epsilon-1) \cdot N}
        > \frac{\frac{1-\epsilon}2 (C_\epsilon-1) \cdot C_\epsilon^{2y}}{C_\epsilon^{2y+1}}
        \ge \frac{1-\epsilon}2 \cdot \frac{\frac1\epsilon-2}{\frac1\epsilon-1}
        \ge \frac{1-\epsilon}2 \cdot \frac{1-2\epsilon}{1-\epsilon}
        = \frac12 - \epsilon.
    \]
    Otherwise, if Alice outputs the wrong value, since Bob terminates first, at least $\frac12$ of Bob's message $\hat{y}_y$ (which should've been all $\emptyset$'s) are actually $0$'s. Then, the adversary corrupted at least 
    \[
        \frac{\frac12 C_\epsilon^{2y+1} N}{(C_\epsilon^{2y+1}-1)/(C_\epsilon-1) \cdot N}
        \ge \frac{C_\epsilon-1}2
        = \frac{1}{2\epsilon}-1 
        > \frac12 - \epsilon
    \]
    for all $\epsilon \le \frac12$ (which is the range we are concerned with). 
    \end{itemize}
\end{proof}

In fact, a noise resilience of $\frac12$ is optimal in the first termination model. The proof of \cite{AgrawalGS16} that $\xi_0 \le \frac12$ easily extends to an upper bound of $\xi_1$ by $\frac12$ as well: An adversary can corrupt every other of Alice's messages so that Bob alternatingly receives messages computed as if Alice's input is $0$ or as if Alice's input is $1$. The adversary can do the same for Bob's messages. Then, when the first party terminates, that party cannot tell if the other party's input was $0$ or $1$. Note that if we compute the noise rate relative to the first termination, we get a noise rate of $\frac12$. This shows that $\xi_1 \le \frac12$.

\begin{theorem}[Corollary of Theorem 5.5 in~\cite{AgrawalGS16}]
    The message exchange protocol is not resilient to a $\frac12$ rate of noise in the first termination model.
\end{theorem}

As a result, we conclude that $\xi_1 = \frac12$.

\begin{theorem}
    $\xi_1 = \frac12$.
\end{theorem}


==> 2term/2.7-construction.tex <==
\subsection{$2/7$ Construction}

\rnote{We define $\DEC(c)$ to be $x$ such that $\Delta(\ECC(x), c)$ is minimal. }

\protocol{Scheme with Resilience $\frac27$ in the Second Termination Model}{2/7}{
    \begin{enumerate}\setcounter{enumi}{-1}
    \item 
        Alice and Bob decide on a family of codes $\ECC_i : \{ 0, 1 \}^{n_A} \rightarrow \Sigma^{N_i}$, with $|\Sigma| = O(1)$. Each $\ECC_i$ has a relative distance of $1 - \epsilon$, where $\epsilon \le \frac{1}{12}$, and length $N_i = i$. Furthermore, $\ECC_i(x)$ is a prefix of $\ECC_j(x)$ for any $i < j$.
    \item 
        Alice encodes $x$ with $\ECC_{N}$ of length $N$ and sends the encoding $\hat{x}$ to Bob.
    \item 
        Bob receives word $\hat{x}$ and computes $t = \Delta(\hat{x}, \ECC_N(\DEC(\hat{x}))$. If $t \ge \frac{1-\epsilon}{2} \cdot N$, he terminates. Otherwise, let 
        \[
            L = \begin{cases}
                \frac{4N}3 - 2t & 0 \le t < \frac{N}3 \\
                2N - 4t & \frac{N}3 \le t < \frac{1-\epsilon}2 \cdot N.
            \end{cases}
        \]
        Bob sends Alice $\ECC_L(y)$. 
    \item 
        After Bob finishes sending $\ECC_L(y)$, he outputs $(\DEC(\hat{x}), y)$ and terminates.
    \item 
        Alice keeps listening either until round $N + \frac{4N}3$, or until she has received $\frac{2N}3$ (not necessarily consecutive) $\emptyset$'s, whichever comes first. She then terminates and outputs $(x, \DEC(\hat{y}))$, where $\hat{y}$ is all the bits she has received.
    \end{enumerate}

}

\begin{theorem}
    Protocol~\ref{prot:2/7} is resilient to a $(\frac27-\epsilon)$-fraction of noise relative to the second termination.
\end{theorem}
\begin{proof}
    Suppose that the adversary corrupts the communication so that Bob's output is not $(x, y)$. This means that the adversary corrupted $(1-\epsilon) \cdot N - t$ of Alice's bits. If $t < \frac{N}3$, Alice terminates on or before round $N + \frac{4N}3 = \frac{7N}3$, so the adversary corrupted greater than $\frac{(\frac23 - \epsilon)N}{7N/3} = (\frac27 - \frac{3\epsilon}7)N$ of the bits. Otherwise, if $t \ge \frac{N}3$, suppose Alice terminates after $N + (2N - 4t) + \frac{2N}3 + \delta = \frac{11N}3 - 4t + \delta$ rounds. The adversary must've corrupted an additional $\ge |\delta|$ of Bob's messages, for a total corruption rate of 
    \[
        \ge \frac{(1 - \epsilon)N - t + |\delta|}{\frac{11N}3 - 4t + \delta}
        \ge \frac{(1-\epsilon)N - t + |\delta|}{\frac{11N}3 - 4t + |\delta|}
        \ge \frac{(1-\epsilon)N - t}{\frac{11N}3 - 4t}
        \ge \frac{(1-\epsilon)N - \frac{N}3}{\frac{11N}3 - 4 \cdot \frac{N}3}
        = \frac{\frac23 - \epsilon}{\frac73}
        = \frac27 - \frac{3\epsilon}7.
    \]
    \rnote{need epsilon < 1/12}
    
    Next, suppose that the adversary corrupted the communication so that Alice's output is not $(x, y)$. Then either Alice terminates before Bob, or she terminates after Bob. If she terminates before Bob, then the adversary must've corrupted $\frac{2N}3$ of Bob's messages to $\emptyset$'s. Meanwhile, Bob terminates by round $N + \frac{4N}3$, for a total error rate of $\ge \frac{2N/3}{7N/3} = \frac27$. On the other hand, if Alice terminates after Bob, then in the case that $t < \frac{N}3$, she terminates by round $N + \frac{4N}3$. The adversary must've corrupted at least $\frac{1-\epsilon}2 \cdot (\frac{4N}3 - 2t)$ of Bob's messages in order for Alice to learn the wrong value of $y$. This gives a corruption rate of
    \[
        \ge \frac{t + \frac{1-\epsilon}2 \cdot (\frac{4N}3 - 2t)}{\frac{7N}3}
        = \frac{(1-\epsilon) \cdot \frac{2N}3 + \epsilon \cdot t}{\frac{7N}3}
        \ge \frac27 - \frac{2\epsilon}7.
    \]
    Finally, in the case that Alice terminates after Bob and $t \ge \frac{N}3$, suppose Alice terminates in round $N + (2N - 4t) + \frac{2N}3 + \delta = \frac{11N}3 - 4t + \delta$. Then, the adversary must've corrupted at least $\frac{1-\epsilon}2 \cdot (2N - 4t + |\delta|)$ of Bob's messages. This gives a corruption rate of 
    \begin{align*}
        \ge \frac{t + \frac{1-\epsilon}2 \cdot (2N - 4t + |\delta|)}{\frac{11N}3 - 4t + \delta}
        &\ge \frac{t + \frac{1-\epsilon}2 \cdot (2N - 4t + |\delta|)}{\frac{11N}3 - 4t + |\delta|} \\
        &\ge \frac{(1-\epsilon) \cdot N - (1-2\epsilon) \cdot t}{\frac{11N}3 - 4t} \\
        &\ge \frac{(1-\epsilon)\cdot N - (1-2\epsilon)\cdot \frac{N}3}{\frac{11N}3 - 4 \cdot \frac{N}3} \\
        &= \frac{\frac23 - \frac{\epsilon}3}{\frac73} \\
        &= \frac27 - \frac\epsilon7.
    \end{align*}
\end{proof}

==> 2term/ABA-upper-bound.tex <==
\begin{theorem}
    No 2term protocol where the order of speaking goes Alice, Bob, Alice, and both Alice and Bob terminate in the last segment is resilient to something like $1/3-0.01$ noise.
\end{theorem}

\begin{proof}
(copy pasted from notepad, only a sketch, but correct)
Adversary corrupts Alice so she sends 1-2a x0, a x1, a x2.

Case 1: Adversary corrupts Bob so he sends 0.5 y0, 0.5 y1 when he either of the two

Wlog Alice guesses y0 from this, if bob actually has y1 and Alice x0, the protocol needs to terminate by 6a. (Let Bobs guess be k though it doesn’t matter yet). Another consequence of this is that if Bob hears any 15a bits, followed by 36a term bits, he must terminate.

Case 2: adversary doesn’t corrupt Bob, bob has y1.

Wlog, x1 != k (wlog is over x1, x2). If Alice has x1, and the adversary employs this attack, and then corrupts 6a Alice bits at the end to simulate the previous case occurring, bob will guess wrong, so the protocol needs to terminate by 15a, specifically Alice needs to stop talking by 15a.

However if the adversary doesn’t corrupt anything, bob needs to, after hearing the 15a correct bits (and possibly more termination bits), guess x1.

But if Alice actually has x0, upon hearing 15a bits from above and 36a term bits, she must have terminated by then as shown way above. She has to guess x1, but if Alice actually had x1, the adversary just corrupts all 51a of these bits, and has only corrupted 53a bits total, and deceived a party.
    
\end{proof}

\begin{theorem}[False theorem]
    No adaptive termination protocol where all of Bob's rounds are contiguous and Alice and Bob both terminate after all of Bob's rounds is resilient to a $\frac{1}{1+\sqrt5}$ fraction of noise relative to the second termination.
\end{theorem}

\begin{proof}
    Suppose in the protocol, Alice talks for $N$ rounds, then Bob speaks for $L$ rounds, and then Alice speaks for some more rounds. Consider a run of the protocol where the adversary first corrupts half of Alice's first $N$ bits so that half of the $N$ messages are as if she had $x_0$, and the other half are as if she had $x_1$. 
    
    Consider the following scenarios:
    \begin{itemize}
        \item 
            First, suppose that the adversary corrupts Bob's messages so that $(\frac12 + \frac{N}{4L}) \cdot L$ of the messages are as if Bob had seen half $x_0$, half $x_1$, and the other $(\frac12 - \frac{N}{4L})\cdot L$ are as if Bob had seen all $x_0$. I wanted to claim that Bob has to terminate by $\phi$, so you get $\frac{L/2 + N/4}{N + L + \phi}$, but the fact is that Bob can terminate later if sees half and half than if sees just $x_0$ ... this case is messed up
        \item 
            Note that if Bob gets half and half, and Alice gets Bob's honest messages, and if she talks $M$, then the adversary can corrupt half of the remaining to get $\frac{N/2 + M/2}{N + L + M}$. Also, you can force Bob to terminate early, so $\frac{N/2 + \phi}{N + L + M}$.
    \end{itemize}
    
    I think I messed up. I wanted $\frac{L/2 + N/4}{N + L + \phi}$, $\frac{N/2 + \phi}{N + L + M}$, $\frac{(N + M)/2}{N + L + M}$, which gives $\frac12 - \frac{\sqrt{k+2}-1}{2(k+1)}$ where $k = N / L$. Then, using the attack where you corrupt half of Bob's bits, you compare this to $\frac{L/2}{N+L}$ and get that it has to be $\frac{1}{\sqrt5 + 1}$. But alas.
\end{proof}

